Maintaining Expander Decompositions via Sparse Cuts

In this article, we show that the algorithm of maintaining expander decompositions in graphs undergoing edge deletions directly by removing sparse cuts repeatedly can be made efficient. Formally, for an $m$-edge undirected graph $G$, we say a cut $(S, \overline{S})$ is $\phi$-sparse if $|E_G(S, \overline{S})| < \phi \cdot \min\{vol_G(S), vol_G(\overline{S})\}$. A $\phi$-expander decomposition of $G$ is a partition of $V$ into sets $X_1, X_2, \ldots, X_k$ such that each cluster $G[X_i]$ contains no $\phi$-sparse cut (meaning it is a $\phi$-expander) with $\tilde{O}(\phi m)$ edges crossing between clusters. A natural way to compute a $\phi$-expander decomposition is to decompose clusters by $\phi$-sparse cuts until no such cut is contained in any cluster. We show that even in graphs undergoing edge deletions, a slight relaxation of this meta-algorithm can be implemented efficiently with amortized update time $m^{o(1)}/\phi^2$. Our approach naturally extends to maintaining directed $\phi$-expander decompositions and $\phi$-expander hierarchies and thus gives a unifying framework while having simpler proofs than previous state-of-the-art work. In all settings, our algorithm matches the run-times of previous algorithms up to subpolynomial factors. Moreover, our algorithm provides stronger guarantees for $\phi$-expander decompositions. For example, for graphs undergoing edge deletions, our approach is the first to maintain a dynamic expander decomposition where each updated decomposition is a refinement of the previous decomposition, and our approach is the first to guarantee a sublinear $\phi m^{1+o(1)}$ bound on the total number of edges that cross between clusters across the entire sequence of dynamic updates.

==> eh.tex <==

\section{Expander Hiearchy}

\rasmus{need to say somewhere that during a vertex split, we are
  allowed to turn self-loops into edges}

\rasmus{needs a little explanatory/padding text}

\begin{definition*}[Induced Graph with Self-Loops]
Let $G[X]^{\tau}$ be the graph $G$ induced by vertex set $X$ where each vertex $v \in X$ receives an additional number of $\lceil \tau \cdot |E(\{x\}, V \setminus X)| \rceil$ self-loops. For a partition $\mathcal{X}$, we denote by $G[\mathcal{X}]^{\tau}$ the union of the graphs $G[X]^{\tau}$ for $X \in \mathcal{X}$.
\end{definition*}

\begin{definition*}[Undirected Boundary-Linked Expander Decomposition]
  Given an \emph{undirected} graph $G$ and parameters $\phi,\alpha \in
  (0,1], \beta > 0$,
  we say that a tuple $(\mathcal{X}, R)$ forms an $(\alpha,\beta,
  \phi)$-expander decomposition
  of $G$ where $\mathcal{X}$ is a partition of $V$ and $R \subseteq E$ if 
(1) for each $X \in \mathcal{X}$, cluster $G[X]^{\alpha/\phi}$ is a $\phi$-expander,
and (2) $R$ is the set of edges not in any cluster and is of size at most $\beta \phi m$.
\end{definition*}

We can derive the following corollary.

\begin{theorem}[Undirected Boundary-Linked Dynamic Expander
  Decomposition]
  \label{thm:bndryLnkdDynED}
  Consider an $m$-edge undirected graph $G$ undergoing a sequence of $O(m)$ updates consisting of edge deletions, vertex splits and self-loop insertions, parameters $\phi \in (0,1)$ and $L_{max} \in \mathbb{N}_{\geq 1}$. 

Then, we can maintain a $(1/\gamma,\gamma, \phi/\gamma)$-expander decomposition
$\mathcal{X}$ for $\gamma = (\log(m))^{5^{O(L_{max})}}$ with the
properties that at any stage (1) the current partition $\mathcal{X}$ is
a refinement of all its earlier versions, and (2) the set $R$ is a
super-set of all its earlier versions. The algorithm takes total time
$m^{1+1/L_{max}}\gamma/\phi^2$ assuming that at most $O(m)$ \rasmus{ok?} self-loops are inserted over the course of the algorithm and succeeds with high probability.
\end{theorem}
\begin{proof}[Proof sketch.]
  We run the Dynamic Expander Decomposition of
  Theorem~\ref{thm:mainTheoremDet} on a copy of $G$ which we denote by $H$.
  When $G$ is changed by a dynamic update, we make the same change to
  $H$.
  But additionally, in $H$, we add self-loops to vertices, whenever an edge incident on the vertex
  enters $R$.
  We call these \emph{regularizing self-loops}.
  
  When a new edge $e$ enters $R$, for each of its endpoints $u$,
  let $R_u$ be the set of edges in $R$ incident of $u$, and let $s_u$
  be the number of regularizing self-loops placed on $u$ in so far.
  If $|R_u|\cdot \frac{1}{\phi}  > s_u$, we add additional
  regularizing self-loops to $u$ until this is no longer the case.
  Note that adding these self-loops may cause further changes to the
  partition, which may in turn cause additional edges to be added to
  $R$, and this may require us to add yet more regularizing
  self-loops. However, in a moment, we will argue that this process
  does not create too many cut edges.
  First, though, let us observe that for each $X \in \mathcal{X}$,
  the regularizing self-loops precisely ensures that $G[X]^{\frac{1}{\phi}} = H[X]$ is
  a $\frac{\phi}{\gamma}$-expander with boundary-linkedness
  parameter $\alpha = \frac{1}{\gamma}$.

  Finally, we need to argue that the addition of regularizing
  self-loops does not mean that we cut too many edges.
  The underlying guarantee of \Cref{thm:mainTheoremDet} guarantees
  that starting with $m$ edges, after $O(m)$ updates, we cut at most
  $\phi m$ edges (i.e. put them into $R$).
  However, this implies that we add most
  $2\phi m \cdot \frac{1}{\phi}  = 2m$ regularizing self-loops.
  Thus, the addition of self-loops does not exceed our budget, and still
  leaves us able to receive further $O(m)$ self-loops updates to $G$,
  albeit with a slightly smaller budget.
\end{proof}






In \cite{goranci2021expander}, the notion of an expander hierarchy is
proposed for undirected graphs $G$ undergoing edge insertions and
deletions.
We introduce a very similar, but sligthly more convenient, notion of
expander hierarchy, using terminolgy inspired by \cite{goranci2021expander}.



\begin{definition*}[Undirected Dynamic Expander Hierarchy]
An $(\alpha, \beta, \phi)$-expander hierarchy is recursively
defined to consist of levels $0 \leq i \leq k$ where we have graphs
$G_i$ where $G_0 = G$ and an $(\alpha,\beta, \phi)$-expander decomposition
$\mathcal{X}_i$ of $G_i$ and we define $G_{i+1}$
recursively to be the graph $G$ after contracting the sets in the
expander decomposition $\mathcal{X}_{i+1}$ \rasmus{should contraction
  remove or retain self-loops?}, and finally have that
$G_k$ consists of only a single vertex.
\end{definition*}

\begin{theorem}

    Consider an $m$-edge undirected graph $G$ undergoing a sequence of $O(m)$ updates consisting of edge deletions, vertex splits and self-loop insertions, parameters $\phi \in (0,0.99)$ and $L_{max} \in \mathbb{N}_{\geq 1}$. 
We can maintain a 
  $(1/\gamma, \gamma, \phi/\gamma)$-expander hierarchy with $k =
  \log_{\frac{1}{\phi}}(m) + 1$ levels with total update time
  $O(m^{1+1/L_{max}}\gamma/\phi^2)$.
  The algorithm works against an adaptive adversary and succeeds with
  high probability.
\end{theorem}

\begin{proof}[Proof sketch.]
  We construct the dynamic expander hierarchy as follows:
  
  We construct the dynamic
  expander decomposition of $G_i$ at each level using
  \Cref{thm:bndryLnkdDynED}.
  When a partition gets refined at level $i$, this corresponds to a
  vertex in level $i+1$ splitting into two, with edges resulting
  betweem.
  We can maintain the
  graph at level $i+1$ by first inserting self-loops on the vertex
  corresponding to the vertex which is about to split, and then
  splitting the vertex while turning the self-loops into edges between
  the vertices.
  
  By the guarantees of this theorem, using induction on the level
  $i$, we can directly show that $G_i$ has at most $\phi^i m$ edges
  initially, and receives at most $O(m)$
  updates, all of the forms allowed by \Cref{thm:bndryLnkdDynED}.

  At level $k = \log_{1/\phi}(m)+1$, we have $<1$ edge left,
  and so the graph must be a single vertex.
  The running time to maintain level $0$ is
  $O(m^{1+1/L_{max}}\gamma/\phi^2)$, and it decays geometrically
  across levels, so the remaining levels only add another constant
  factor.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:
